DeepBern-Nets: Taming the Complexity of Certifying Neural Networks using Bernstein Polynomial Activations and Precise Bound Propagation

Formal certification of Neural Networks (NNs) is crucial for ensuring their safety, fairness, and robustness. Unfortunately, on the one hand, sound and complete certification algorithms of ReLU-based NNs do not scale to large-scale NNs. On the other hand, incomplete certification algorithms are easier to compute, but they result in loose bounds that deteriorate with the depth of NN, which diminishes their effectiveness. In this paper, we ask the following question; can we replace the ReLU activation function with one that opens the door to incomplete certification algorithms that are easy to compute but can produce tight bounds on the NN's outputs? We introduce DeepBern-Nets, a class of NNs with activation functions based on Bernstein polynomials instead of the commonly used ReLU activation. Bernstein polynomials are smooth and differentiable functions with desirable properties such as the so-called range enclosure and subdivision properties. We design a novel algorithm, called Bern-IBP, to efficiently compute tight bounds on DeepBern-Nets outputs. Our approach leverages the properties of Bernstein polynomials to improve the tractability of neural network certification tasks while maintaining the accuracy of the trained networks. We conduct comprehensive experiments in adversarial robustness and reachability analysis settings to assess the effectiveness of the proposed Bernstein polynomial activation in enhancing the certification process. Our proposed framework achieves high certified accuracy for adversarially-trained NNs, which is often a challenging task for certifiers of ReLU-based NNs. Moreover, using Bern-IBP bounds for certified training results in NNs with state-of-the-art certified accuracy compared to ReLU networks. This work establishes Bernstein polynomial activation as a promising alternative for improving NN certification tasks across various applications.

==> figs/NN.tex <==
\begin{tikzpicture}[x=2.2cm,y=1.4cm]
  \message{^^JNeural network, shifted}
  \readlist\Nnod{3,4,4,4,4,3} % array of number of nodes per layer
  \readlist\Nstr{n,m,m,m,m,k} % array of string number of nodes per layer
  \readlist\Cstr{\strut y^0,y^{1},\sigma,y^{2},\sigma,y^3} % array of coefficient symbol per layer
  \def\yshift{0.5} % shift last node for dots
  
  \message{^^J  Layer}
  \foreachitem \N \in \Nnod{ % loop over layers
    \def\lay{\Ncnt} % alias of index of current layer
    \pgfmathsetmacro\prev{int(\Ncnt-1)} % number of previous layer
    \message{\lay,}
    \foreach \i [evaluate={\c=int(\i==\N); \y=\N/2-\i-\c*\yshift;
                 \index=(\i<\N?int(\i):"\Nstr[\lay]");
                 \x=\lay; \n=\nstyle;}] in {1,...,\N}{ % loop over nodes
      % NODES
      \node[node \n] (N\lay-\i) at (\x,\y) {$\Cstr[\lay]_{\index}$};
      
      % CONNECTIONS
      \ifnum\lay>1 % connect to previous layer
        \foreach \j in {1,...,\Nnod[\prev]}{ % loop over nodes in previous layer
          \draw[connect,white,line width=1.2] (N\prev-\j) -- (N\lay-\i);
          \draw[connect] (N\prev-\j) -- (N\lay-\i);
          %\draw[connect] (N\prev-\j.0) -- (N\lay-\i.180); % connect to left
        }
      \fi % else: nothing to connect first layer
      
    }
    \path (N\lay-\N) --++ (0,1+\yshift) node[midway,scale=1.5] {$\vdots$};
  }
  
  % LABELS
    \node[above=5,align=center,black] at (1,-4.0) {Input\\[-0.2em]layer};
    \node[above=2,align=center,black] at (2,-0.5) {Linear\\[-0.2em]layer};
    \node[above=10,align=center,black] at (3,-8.45) {Bernstein\\[-0.2em]activation};
    \node[above=2,align=center,black] at (4,-0.5) {Linear\\[-0.2em]layer};
    \node[above=10,align=center,black] at (5,-8.45) {Bernstein\\[-0.2em]activation};
    \node[above=10,align=center,black] at (6,-9.0) {Output\\[-0.2em]layer};

  
\end{tikzpicture}

==> figs/bern_activation.tex <==
 \begin{tikzpicture}[rotate=90]
    \node [](x) at (0,4.5) {\large $x$};
    

    \node [circle,draw=black,fill=white,inner sep=0pt,minimum size=0.6cm] (u1) at (-1.5,2.0) { $b_{n,0}^{[l,u]}(x)$};
    % \node [circle,draw=black,fill=white,inner sep=0pt,minimum size=0.6cm] (u2) at (-0.5,2.0) { $b_{n,1}^{[l,u]}(x)$};
    \node [circle,draw=black,fill=white,inner sep=0pt,minimum size=0.6cm] (u3) at (1.5,2.0) { $b_{n,n}^{[l,u]}(x)$};

    % \node[mark size=1pt,color=black] at (-0.5,2.0) {\pgfuseplotmark{*}};
    \node[mark size=1pt,color=black] at (-0.3,2.0) {\pgfuseplotmark{*}};
    \node[mark size=1pt,color=black] at (-0.1,2.0) {\pgfuseplotmark{*}};
    \node[mark size=1pt,color=black] at (0.1,2.0) {\pgfuseplotmark{*}};
    \node[mark size=1pt,color=black] at (0.3,2.0) {\pgfuseplotmark{*}};
    % \node[mark size=1pt,color=black] at (0.5,2.0) {\pgfuseplotmark{*}};


    \node [circle,draw=black,fill=white,minimum size=0.65cm] (y) at (0,0.0) {\large $\Sigma$};
    \node [] (out) at (0,-2.8) {\large $\sigma(x;l,u,c_0,...,c_n)$};
    
    \coordinate[] (start) at (0.0,3.8) {};

    \node [rectangle,draw=black,fill=pink,text width=0.5cm] (c0) at (0.0,3.0) {$l,u$};
    % \node [text width=0.5cm] (c3) at (1.5,3.5)  {$l,u$};
    
    % \node [text width=0.5cm] (a0) at (2.5,2.6) {$\alpha,\beta$};
    % \node [circle,draw=black,fill=white,inner sep=0pt,minimum size=0.65cm] (tau_epsilon) at (2.5,1.6) {\large $\tau_{\epsilon}$};
    
    \path [draw,->,anchor=west] (u1) edge node {$c_0$} (y) ;
    \path [draw,->,anchor=west] (u3) edge node {$c_n$} (y);
    % \path [draw] (x.0) edge[->] (u1) edge[->] (u3);
    \path [draw] (start.0) edge[->] (u1) edge[->] (u3);
    \path [draw,-] (x) edge (start);
    % \draw[->] (x) -- (intersection cs: first line={(x)--(u1)}, second line={(x)--(u3)});
    \path [draw,->] (c0) edge (u1);
    \path [draw,->] (c0) edge (u3);
    % \path [draw,->] (c3) edge (u3);
    \path [draw,->] (y) edge (out);


    % \path [draw,->] (c0) edge (lambda);
    % \path [draw,->] (tau_epsilon) edge (x);
    % \path [draw,->] (a0) edge (tau_epsilon);
    % \plate [color=red] {part1} {(x)(u1)} { };
    \plate [color=blue] {part3} {(y)(u1)(u3)(c0)(start)} { };

    % \node [text width=2cm] at (-0.6,-0.5) {\large $n_1$};
    % \node [text width=2cm] at (2,-0.5) {\large $n_d$};

    \end{tikzpicture}

